Towards a Lightweight Multi-Cloud DSL for Elastic and Transferable Cloud-native Applications

Cloud-native applications are intentionally designed for the cloud in order to leverage cloud platform features like horizontal scaling and elasticity - benefits coming along with cloud platforms. In addition to classical (and very often static) multi-tier deployment scenarios, cloud-native applications are typically operated on much more complex but elastic infrastructures. Furthermore, there is a trend to use elastic container platforms like Kubernetes, Docker Swarm or Apache Mesos. However, especially multi-cloud use cases are astonishingly complex to handle. In consequence, cloud-native applications are prone to vendor lock-in. Very often TOSCA-based approaches are used to tackle this aspect. But, these application topology defining approaches are limited in supporting multi-cloud adaption of a cloud-native application at runtime. In this paper, we analyzed several approaches to define cloud-native applications being multi-cloud transferable at runtime. We have not found an approach that fully satisfies all of our requirements. Therefore we introduce a solution proposal that separates elastic platform definition from cloud application definition. We present first considerations for a domain specific language for application definition and demonstrate evaluation results on the platform level showing that a cloud-native application can be transferred between different cloud service providers like Azure and Google within minutes and without downtime. The evaluation covers public and private cloud service infrastructures provided by Amazon Web Services, Microsoft Azure, Google Compute Engine and OpenStack.

==> sections/implementation.tex <==
 , %!TEX root = ../closer_paper.tex
\section{\uppercase{Implementation}}
\label{sec:implementation}


==> sections/related_work.tex <==
 %!TEX root = ../closer_paper.tex
\section{\uppercase{Related Work}}
\label{sec:related_work}

\noindent According to \cite{Barker2015,Petcu2011,Toosi2014,Grozev2014} there are several promising approaches dealing with multi-cloud scenarios. However, none of these surveys identified elastic container platforms as a viable option. Just \cite{Petcu2014} identified the need to \textit{"adopt open-source platforms"} and \textit{"mechanisms for real-time migration"} at run-time level but did not identifiy (nor integrate)  concrete and existing platforms or solutions. All surveys identified approaches fitting mainly in the following fields: 
\textbf{Volunteer federations} for groups of \textit{"cloud providers collaborating voluntarily with each other to exchange resources"} \cite{Grozev2014}.
\textbf{Independent federations} (or multi-clouds) \textit{"when multiple clouds are used in aggregation by an application or its broker. This approach is essentially independent of the cloud provider"} and focus on the client-side of cloud computing \cite{Toosi2014}.

Our research approach focuses on independent federations (multi-clouds). We do not propose a broker-based solution \cite{Barker2015} because cloud-brokers have the tendency just to shift the vendor lock-in problem to a broker. However, the following approaches show some similarities. The following paragraphs briefly explain how the proposed approach is different.
Approaches like \textbf{OPTIMIS} \cite{Ferrer2012}, \textbf{ConTrail} \cite{Carlini2012}, \textbf{CYCLONE}\cite{demchenko2016cyclone} or \textbf{multi-cloud PaaS  platforms} \cite{Paraiso2012} enable dynamic provisioning of cloud services targeting multi-cloud architectures. These solutions have to provide a lot of plugins to support possible implementation languages. In 2012, Paraiso et al. identified at least 19 different plugins (just for a research prototype) \cite{Paraiso2012} . This increases the inner complexity of such kind of solutions. Container-based approaches might be better suited to handle this kind of complexity.
Approaches like \textbf{mOSAIC} \cite{Petcu2011} or \textbf{Cloud4SOA} \cite{Kamateri2013} assume that an application can be divided into components according to a service oriented application architecture (SOA). These approaches rely on the case that that applications are bound to a specific run-time environment. This is true for the proposed approach as well. However, we investigate a solution where the run-time environment (elastic container platform) is up to a user decision as well.

We found several deployment description languages like \textbf{TOSCA} \cite{binz2014tosca,BSW2014,Binz2014}, \textbf{CAMEL} \cite{Rossini2015} or \textbf{CloudML} \cite{Brandtzaeg2012,lushpenko2015using} and frameworks like \textbf{PaaSage}\footnote{see \url{http://www.paasage.eu/} (last access 22th Aug. 2017)} \cite{Rossini2015} which combine such DSL with runtime environments. 
Nonetheless, this contribution is focused on a more container-centric approach.

All in all, the proposed approach intends to be more \textit{pragmatic}, \textit{lightweight} and \textit{complexity hiding} using existing elastic container platforms. On the downside, it might be only applicable for container-based applications. But to use container platforms gets more and more common in CNA engineering.

==> sections/sme_vendor.tex <==
 %!TEX root = ../closer_paper.tex
\section{\uppercase{SME and Vendor Lock-In} }
\label{sec:sme}

%\textbf{TODO Ggf. Kapitel streichen!}Our research focus is in making cloud computing useable for \textbf{small and medium-sized enterprises} (SME) and \textbf{avoiding vendor lock-in} in cloud-native application deployments.
%
%At first glance, cloud computing has a lot of benefits for SMEs: they can get access to a large scale of computational resources in a fast and easy way. Resources can be requested on demand, investment risk can be reduced by rent instead of buying resources and features like auto-scaling can prevent unnecessary costs \cite{Armbrust2009} when, e.g., a new web service does not have the intended success. On the other hand, if the new service is widely used, there is no danger of service-crash because of inadequate resources.
%
%A major obstacle for SMEs in cloud computing is vendor lock-in \cite{Kra2014a}. To \textbf{avoid vendor lock-in}, our approach is using the very basic  cloud services only  - requesting computational and storage resources in the form of virtual machines. This services are covered by conceptually by standards like OCCI, CIMI, CDMI, etc.). Because of missing standardization of the majority of other offered services, using this services increase the risk of vendor lock-in. To provide features like elasticity, auto-scaling and multi-cloud-deployments, an open source \textbf{elastic container platform} (ECP) such as \textit{Kubernetes}, \textit{Docker Swarm Mode} and \textit{Apache Mesos} can be used. The ECP nodes can be hosted on (virtual) machines provided by IaaS platforms. These machines do not have to be provided by the same IaaS provider. This enables \textbf{hybrid-cloud} and \textbf{multi-cloud environments}.  As shown in Figure \ref{fig:migration}, next to the benefits running a CNA on multi-cloud environments, this architecture type also enables  \textbf{cloud migration}.
%
%\begin{figure*}
%	\begin{center}
%		\includegraphics[width=\textwidth]{img/workflow_migrating.pdf}
%		\caption{Migrating IaaS platform. (1) Cluster hosted on VM by source provider A, (2) extending cluster with machines provided by target provider B, (3) terminating source provider VM, automatical detection and recreation of missing containers on target provider machines. (4) Migration complete.}	
%		\label{fig:migration}
%	\end{center}
%\end{figure*}
%
%However, deploying cloud-native applications in an auto-scaling manner, can be (too) hard to handle for a small company, especially when provider-independency and the possibility of migration are required.
\textbf{TODO Integireren: Kein eigenes Kapitel} Our approach is to \textbf{capsule the inherent complexity} of such a CNA deployment by making use of elastic container platform. Therefore, we developed, a proof-of-concept system which enables an automatic deployment of an elastic platform \cite{Kratzke2016}\cite{Quint2017}. Currently, the system can automatically deploy an autoscaling multi-cloud environment. As elastic container platform Kubernetes is used (the support of further cluster platforms like Docker Swarm Mode and Apache Mesos will follow and is shown by \cite{Kratzke2016}). 

